Tracing the Lifecycle of Architecture Technical Debt in Software Systems: A Dependency Approach

Architectural technical debt (ATD) represents trade-offs in software architecture that accelerate initial development but create long-term maintenance challenges. ATD, in particular when self-admitted, impacts the foundational structure of software, making it difficult to detect and resolve. This study investigates the lifecycle of ATD, focusing on how it affects i) the connectivity between classes and ii) the frequency of file modifications. We aim to understand how ATD evolves from introduction to repayment and its implications on software architectures. Our empirical approach was applied to a dataset of SATD items extracted from various software artifacts. We isolated ATD instances, filtered for architectural indicators, and calculated dependencies at different lifecycle stages using FAN-IN and FAN-OUT metrics. Statistical analyses, including the Mann-Whitney U test and Cliff's Delta, were used to assess the significance and effect size of connectivity and dependency changes over time. We observed that ATD repayment increased class connectivity, with FAN-IN increasing by 57.5% on average and FAN-OUT by 26.7%, suggesting a shift toward centralization and increased architectural complexity after repayment. Moreover, ATD files were modified less frequently than Non-ATD files, with changes accumulated in high-dependency portions of the code. Our study shows that resolving ATD improves software quality in the short-term, but can make the architecture more complex by centralizing dependencies. Also, even if dependency metrics (like FAN-IN and FAN-OUT) can help understand the impact of ATD, they should be combined with other measures to capture other effects of ATD on software maintainability.

==> old/overall_results.tex <==
\subsection{Overall results}

% \subsection{ATD item of CAMEL-789}
% When analyzing the ATD item from Jira issue tracker with issue ID CAMEL-789\footnote{https://issues.apache.org/jira/browse/CAMEL-789}, which has the description: \textit{"When downloading artifacts, we have many repos. Several of them are specific for a single/few components. We should move these repo settings to these targeted components and let the uber pom.xml have only the major public maven repos. Maybe some of the repos are out-of-date and not used anymore,"} this issue was resolved with commit hashcode \#8c56ead\footnote{https://github.com/apache/camel/commit/8c56ead7e728550c0f086e51070c7a5973cc28aa}. This commit resulted in changes to 15 files, with 117 additions and 95 deletions. These changes were made by a single developer on August 7, 2008.

% Tracing back to the introduction of this ATD, it was found that it began on March 19, 2007, with commit hashcode \#77b260b\footnote{https://github.com/apache/camel/commit/77b260b65ba821b3443d922320cc3d9b708c8d83}. This ATD was introduced when a different developer made changes to 42 files with 2,295 additions, one of which was "camel/camel-core/pom.xml". 

% The interval between the introduction and payment of this ATD spanned 507 days. During this period, the payment process significantly altered the dependency graph. Initially, at the phase of introduction, the graph had 33 nodes, 84 links and 8 leaf nodes. By the time the issue was resolved, it had grown to 979 nodes, 4,229 links and 127 leaf nodes.


% \subsection{ATD item of CAMEL-4357}

% \subsection{ATD item of HADOOP-6374}
% ...\\



%\subsection{How does the size of a dependency graph correlate with the effort required to repay architecture technical debt?}
\subsubsection{How does architectural technical debt affect the connectivity of classes within the software system?}

To investigate how ATD affects the connectivity of classes in the software system, we conducted a comparative analysis of the ATD at two key stages: its introduction and its payment. First, we began with a set consisting of 34 out of 116 ATD items, which were unanimously identified as genuine ATD items by all authors of this study. In the issue section dataset, we found that 10 out of 22 items did not have corresponding issue IDs in the repository commits. Similarly, 2 out of 3 items lacked commit hashcodes in the pull section dataset in the repository. Consequently, the total number of ATD items available from all artifacts for further study is 12 from the issue section, 1 from the pull section and 9 from the commit messages.

The aim of this analysis is to explore whether the presence of ATD increases or decreases the complexity of the software, measured by changes in connectivity between classes. This is evaluated through the FAN-IN and FAN-OUT metrics \cite{mubarak2010evolutionary}, which reflect how many classes depend on or are used by the classes associated with the ATD in the phase of its introduction and payment. The FAN-IN and FAN-OUT values at the introduction and payment moments for ATD items are compared to assess how the architecture evolved over time. By comparing the results, the study aims to uncover the potential impact of ATD on increasing dependencies and complexity within the software system.

Instead of calculating the dependencies for the entire project, we chose to focus only on the files directly involved in the commits related to ATD. This decision was made after initially considering a broader analysis of the whole project. However, analyzing the entire project proved to be ineffective, as it produced overly complex and non-specific dependency data. Since not all files in the project are affected by ATD, including unrelated files in the analysis led to a lack of focus and unnecessary complexity. By narrowing our focus to the files specifically impacted by ATD-related commits, we were able to gain more profound and relevant insights into how ATD influences connectivity and dependencies in the system’s critical components.

For the 22 identified ATD items, we calculated the FAN-IN and FAN-OUT values at two crucial points: the introduction phase, when the ATD was first identified and the payment phase, when the ATD was resolved. These calculations were carried out using Understand by SciTools \cite{scitools2024}, which provided detailed insights into the dependencies between classes at both stages. During the introduction phase, we compiled a comprehensive list of all the files involved, along with their file paths and calculated their dependency values (FAN-IN and FAN-OUT). The same analysis was repeated for the payment phase, focusing on the same files that were identified during the introduction.

To ensure accuracy in comparing the two phases, we used the \texttt{git checkout} command with the appropriate commit hash code to retrieve the exact state of the code at both the introduction and payment phases. This approach allowed us to directly assess the evolution of the dependencies and how the connectivity between classes was affected by the presence and resolution of ATD over time. 

PyDriller \cite{PyDriller} was used to identify whether the files involved in a commit had undergone changes, been renamed, moved, or were deleted. We tracked all these files during the payment interval for each ATD item, with PyDriller tracing the last known location of each file to capture any modifications or relocations.

In this analysis, we focused solely on files that were changed, renamed, or moved during this period. Files initially present in the introduction phase but later deleted were excluded from the analysis. Files that were present in the introduction phase but later deleted were excluded from consideration, as deletions often result from refactoring or the resolution of the ATD itself \cite{tom2013exploration}. By excluding these files, we ensured that the analysis targeted the ongoing impact of ATD on the system and avoided conflating ATD resolution with unrelated structural changes.

To assess how ATD affects overall system connectivity, average values of FAN-IN and FAN-OUT are used to capture broad trends across the system. By analyzing the average changes in these values from the moment ATD is introduced to the time it is paid off, we can measure the extent to which ATD impacts the relationships between system components.


\begin{table}[h]
\centering
\caption{FAN-IN and FAN-OUT Changes of ATD}
\begin{tabular}{cccc}
\toprule
Metric & Introduction & Payment & Percentage Increase\\
\midrule
Number of files & 5,135 & 3,553 & -44.5\%\\
Avg. FAN-IN  & 8.03  & 18.89  & 57.5\%  \\ %\hline
Avg. FAN-OUT & 8.09   & 11.04  & 26.7\%  \\ %\hline
Max. FAN-IN & 1,360 & 2,684 & 97.35\% \\
Max. FAN-OUT & 235 & 299 & 27.23\% \\ \hline

\end{tabular}
\label{tab:tb_average}
\end{table}



Table~\ref{tab:tb_average} shows the changes in FAN-IN and FAN-OUT metrics between the introduction and payment of ATD. The first row indicates a significant decrease in the number of files, from 5,135 at ATD introduction to 3,553 at payment, a reduction of 44.5\%. Such a reduction might indicate refactoring efforts, consolidation of the codebase, or the removal of obsolete or redundant files during the resolution of technical debt.

The average FAN-IN value at the time of ATD introduction was 8.03, while at the time of ATD payment, it increased to 18.89. This represents a rise of approximately 57.5\% in the number of incoming dependencies after ATD was resolved. The increase in FAN-IN suggests that after ATD payment, classes tend to become more central in the system, with other parts of the system increasingly relying on these classes. This growth in FAN-IN highlights a tendency for certain classes to take on more responsibilities, which could lead to potential architectural bottlenecks or future maintenance challenges as more parts of the system come to depend on these files.

Similarly, the average FAN-OUT value at the time of ATD introduction was 8.09, which increased to 11.04 at the time of ATD payment, representing a 26.7\% increase in outgoing dependencies. Although the growth in FAN-OUT is less dramatic compared to FAN-IN, it still indicates that after ATD resolution, classes tend to form more dependencies with other parts of the system. This may suggest a higher level of coupling, where classes become more interconnected, potentially making the system harder to evolve or refactor in the future.

In addition, the maximum FAN-IN jumped significantly, nearly doubling from 1,360 to 2,684, marking a 97.35\% increase, meaning certain core files gained more dependencies. Meanwhile, the maximum FAN-OUT rose by 27.23\%, from 235 to 299, indicating increased file dependencies.

% \textcolor{red}{\subsubsection{Wilcoxon Signed-Rank Test - WILL BE REMOVED}}
% In our dataset, some files were deleted, or their dependencies were changed between the introduction and payment phases of ATD. As a result, during the payment phase, certain files lack the necessary data for FAN-IN or FAN-OUT values. To handle this, we have substituted these missing values (NA values) with placeholders. This substitution allows us to maintain consistency in the dataset and ensures that the data remains usable for further analysis.

% The decision to use placeholders stems from the fact that once a file is deleted or no longer has any dependencies in the payment phase, its FAN-IN or FAN-OUT effectively becomes zero. Since no other files depend on or are dependent upon the deleted file, there is no connectivity to measure and thus, zero is a reasonable approximation for the missing values. By treating the missing values as zeros, we can perform the Wilcoxon signed-rank test \cite{wilcoxon1992individual} without excluding any data points, which helps in maintaining the integrity of the comparative analysis. This method ensures that we account for all files in ATD items, including those that were removed or modified during the system's evolution.


% FAN-IN values at the point of technical debt introduction and technical debt payment were analyzed using the Wilcoxon Signed-Rank Test \cite{wilcoxon1992individual}. The histogram in Figure~\ref{fig_fan-in} depicts the density distribution of the FAN-IN values, where the blue bars represent the distribution at the time of debt introduction and the red bars show the values at the time of payment. The results indicate a significant reduction in the FAN-IN values after the technical debt was paid, as illustrated by the shift in the distribution. The median FAN-IN at the point of introduction was 2.00, as indicated by the blue dashed line. Meanwhile, after payment, the median FAN-IN dropped to 0.00, represented by the red dashed line.

% %This reduction suggests that the architectural changes leading to the resolution of technical debt resulted in a decrease in the number of incoming dependencies to the affected files or classes, thereby potentially simplifying the system architecture and lowering the overall complexity associated with these components.

% \begin{figure}[htbp!] 
% \centerline{\includegraphics[width=1\textwidth]{figures/fan-in-wilcoxon.pdf}}
% \caption{Density Distribution of FAN-IN}
% \label{fig_fan-in}
% \end{figure}

% Similarly, Figure~\ref{fig_fan-out} illustrates the distribution of FAN-OUT values before and after the payment of technical debt. The blue and red bars represent distributions of FAN-OUT at the introduction and payment points, respectively. The Wilcoxon Signed-Rank Test reveals a significant change in FAN-OUT values after technical debt payment. The median FAN-OUT at the point of introduction was 5.00 (blue dashed line), which decreased to a median of 0.00 (red dashed line) after the technical debt was paid. 

% %The FAN-OUT reduction indicates that fewer classes or components depended on the affected files after the debt was paid, reflecting a decrease in the outward coupling of the system. This reduction in dependencies can be interpreted as a positive architectural change, reducing the propagation of changes and potential ripple effects when modifications are made in the future.

% \begin{figure}[htbp!] 
% \centerline{\includegraphics[width=1\textwidth]{figures/fan-out-wilcoxon.pdf}}
% \caption{Density Distribution of FAN-OUT}
% \label{fig_fan-out}
% \end{figure}

% To evaluate whether these changes were statistically significant, hypothesis testing was conducted using \textit{p}-values. A \textit{p}-value is a statistical measure used to assess whether the observed differences between groups are likely due to chance. A \textit{p}-value less than 0.05 is typically considered statistically significant, meaning that the observed difference is very unlikely to have occurred by random chance. In this study, the \textit{p}-value for FAN-IN was \(6.87 \times 10^{-52}\) and for FAN-OUT it was \(9.28 \times 10^{-202}\), both of which are far below the significance threshold of 0.05. These results confirm that the changes in both FAN-IN and FAN-OUT values between ATD introduction and payment are highly statistically significant.




\subsubsection{Mann-Whitney U Test} 
In our dataset, some files were deleted, or their dependencies were changed between the introduction and payment phases of ATD. As a result, during the payment phase, certain files lack the necessary data for FAN-IN or FAN-OUT values. To handle this, we opted to remove files with missing values altogether. This was done to ensure the accuracy of our analysis, as treating NA values as zeros may not always reflect the true nature of the data. By removing these files, we acknowledge that their FAN-IN or FAN-OUT values cannot be reliably calculated during the payment phase due to deletion or lack of dependencies. However, this removal results in the dataset no longer being paired, as some files present in the introduction phase are missing from the payment phase.

As a consequence, we utilize the Mann-Whitney U Test. This test is appropriate for comparing independent samples, making it a suitable choice for our modified dataset. By using the Mann-Whitney U Test, we can assess the differences in FAN-IN and FAN-OUT values between the introduction and payment phases, while ensuring that the analysis remains statistically sound. This test provides a more conservative and reliable assessment of the data, as it avoids making assumptions deleted files. By focusing only on the files with complete data, we aim to maintain the validity of our comparisons.


The data distribution for FAN-IN and FAN-OUT values is visualized in Figure~\ref{fig_fan-in-out}. These figures depict the log distributions of FAN-IN and FAN-OUT values during the introduction and payment phases of ATD. In Figure~\ref{fig_fan-in-out}, the plot for FAN-IN values shows a clear difference between the two phases. In the introduction phase, the median FAN-IN value is 1.10, while in the payment phase, the median increases to 1.39. This shift in medians suggests an overall increase in FAN-IN values as the ATD is addressed, indicating that files tend to accumulate more inward dependencies when the debt is resolved, implying greater connectivity within the system.

\begin{figure*}[htbp!] 
\centerline{\includegraphics[width=1\textwidth]{figures/merged_atd_in_out.pdf}}
\caption{Distribution of FAN-IN and FAN-OUT : Introduction vs. Payment Phases of ATD}
\label{fig_fan-in-out}
\end{figure*}

Meanwhile, FAN-OUT values at the introduction phase have a median of 1.79, while the median at the payment phase rises slightly to 1.95. Although the increase in FAN-OUT values is subtler compared to FAN-IN, it still indicates a rise in outward dependencies as the system evolves and the ATD is resolved.

The figure employs the Mann-Whitney U Test to compare the two independent samples (introduction vs. payment phases), evaluating whether there is a statistically significant difference between the distributions of FAN-IN and FAN-OUT across the phases. Despite some overlap in the distributions, the shift in medians points to a trend of increasing dependencies—particularly for FAN-IN—during the resolution of technical debt. This suggests that components become more interconnected or central to the system's architecture as ATD is addressed.

The statistical analysis supports these visual observations. The Mann-Whitney U Test for FAN-IN produced a p-value of \(3.05 \times 10^{-20}\), which is far below the typical significance threshold (e.g., 0.05) for a 95\% confidence level. This exceptionally low p-value leads us to reject the null hypothesis that there is no difference between the FAN-IN values during the introduction and payment phases. The shift in medians, as demonstrated in Figure~\ref{fig_fan-in-out}, highlights that the connectivity of files in terms of FAN-IN significantly increases once the ATD is paid off.

% \begin{figure*}[htbp!] 
% \centerline{\includegraphics[width=1\textwidth]{figures/all_data_fan_out_log_transformation.pdf}}
% \caption{Distribution of FAN-OUT: Introduction vs. Payment Phases of ATD}
% \label{fig_fan-out-mann}
% \end{figure*}

\begin{figure*}[htbp!] 
\centerline{\includegraphics[width=1\textwidth]{figures/merged_non_atd_in_out.pdf}}
\caption{Distribution of FAN-IN and FAN-OUT : Initial Commit vs Recorded Phases of Non-ATD }
\label{fig_fan-in-out}
\end{figure*}


% \begin{figure*}[htbp!] 
% \centerline{\includegraphics[width=1\textwidth]{figures/non_atd_all_data_fan_in_log_transformation.pdf}}
% \caption{Distribution of FAN-IN: Introduction vs. Payment Phases of Non-ATD}
% \label{fig_non_atd_in}
% \end{figure*}

% \begin{figure*}[htbp!] 
% \centerline{\includegraphics[width=1\textwidth]{figures/all_data_fan_out_log_transformation.pdf}}
% \caption{Distribution of FAN-OUT: Introduction vs. Payment Phases of Non-ATD}
% \label{fig_non_atd_out}
% \end{figure*}





% \begin{figure*}[htbp!] 
% \centerline{\includegraphics[width=0.8\textwidth]{figures/boxplot_fan-in_atd_non-atd.pdf}}
% \caption{Boxplot of FAN-IN ATD vs Non-ATD}
% \label{fig_fboxplot_fan-in_atd_non-atd}
% \end{figure*}

% \begin{figure*}[htbp!] 
% \centerline{\includegraphics[width=0.8\textwidth]{figures/boxplot_fan-out_atd_non-atd.pdf}}
% \caption{Boxplot of FAN-OUT ATD vs Non-ATD}
% \label{fig_boxplot_fan-out_atd_non-atd}
% \end{figure*}


For FAN-OUT, the Mann-Whitney U Test yielded a p-value of \(1.23 \times 10^{-15}\), also indicating a statistically significant difference at the 95\% confidence level. While the change in median FAN-OUT values, as shown in Figure~\ref{fig_fan-in-out}, is less pronounced than for FAN-IN, the low p-value suggests that the difference is still meaningful. This implies that outward dependencies also tend to rise as ATD is resolved, although to a lesser extent compared to inward dependencies.

These results suggest that although the ATD items have been paid off, resolving ATD can lead to increased connectivity within the system. The significant rise in FAN-IN values points to a growth in inward dependencies, potentially indicating that some files become more central to the system's architecture even as ATD is addressed. The increase in FAN-OUT values, though smaller, suggests a similar trend for outward dependencies. This further underscores the evolving complexity and interconnectivity of the system, where addressing technical debt does not necessarily simplify the architecture but may instead shift and redistribute dependencies across components.


\subsubsection{Cohen’s \textit{d}}
In fact, while \textit{p}-values confirm the statistical significance of these changes, they do not convey the magnitude or practical significance of the differences. In addition to the Wilcoxon Signed-Rank Test and Mann-Whitney U Test, we calculated the effect size using Cohen’s \textit{d} to assess the magnitude of the change in FAN-IN and FAN-OUT values between the technical debt introduction and payment phases. Cohen’s \textit{d} helps quantify the size of the effect: 0.2 indicates a small, noticeable difference; 0.5 reflects a moderate, meaningful difference; and 0.8 or higher represents a large, substantial difference. 

\[
d = \frac{\bar{X}_1 - \bar{X}_2}{s_p}
\]
% \[
% s_p = \sqrt{\frac{(n_1 - 1)s_1^2 + (n_2 - 1)s_2^2}{n_1 + n_2 - 2}}
% \]


The difference in FAN-IN values between the introduction and payment phases of ATD yielded a Cohen’s \textit{d} of -0.2. This value represents a small effect size, suggesting that although there is a statistically significant increase in FAN-IN, the magnitude of the change is modest. In practical terms, this means that while some files became more central to the system's architecture as ATD was resolved, the overall shift in inward dependencies is not substantial enough to indicate a major architectural transformation. The system's connectivity increased, but the effect on architectural cohesion and complexity due to FAN-IN changes is limited.

Similarly, the difference in FAN-OUT values between the introduction and payment phases resulted in a Cohen’s \textit{d} of -0.2, also indicating a small effect size. This suggests that the increase in outward dependencies (FAN-OUT) during the ATD payment phase is similarly modest. While there is a measurable change in the number of outward connections between components, this change does not reflect a significant shift in the system's overall architectural complexity. The rise in FAN-OUT highlights some redistribution of dependencies, but its practical impact remains limited.

Both Cohen’s d scores for FAN-IN and FAN-OUT demonstrate that the differences in connectivity between the introduction and payment phases are small in terms of their practical significance. Although statistically significant, the shifts in inward (FAN-IN) and outward (FAN-OUT) dependencies represent minor adjustments in the system’s architecture rather than large-scale changes. This suggests that while resolving ATD may lead to slight increases in complexity or connectivity, these changes are generally manageable and do not drastically alter the system's architectural structure.



%Similarly, for the 22 non-TD items, FAN-IN and FAN-OUT values were calculated at the time of the first commit and at the recorded time of observation. This enabled a direct comparison with the ATD items to understand whether technical debt influenced the increase or decrease in class dependencies over time.




%After that, we used The Map Equation to create community detection. This method allowed us to effectively identify and analyze the structural community of dependencies during these three phases. Additionally, we recorded the names of the developers involved at each of these stages and the corresponding dates.






% %precession, 

% The Map Equation algorithm works by minimizing the length of the path description followed by random explorers in the network. Random explorers moving within the network tend to spend more time within one community before moving to another community and Huffman coding principles are used to efficiently code the movements of these explorers. In the initial stage, each node is considered a separate community, for example, as depicted in Figure~\ref{fig_bw}, namely the dependency graph from the introduction phase of the Camel project with issue ID CAMEL-789\footnote{https://issues.apache.org/jira/browse/CAMEL-789}.


% \begin{figure}[htbp!] 
% \centerline{\includesvg[width=0.40\textwidth]{bw.svg}}
% \caption{Dependencies graph from introduction phase of CAMEL-789}
% \label{fig_bw}
% \end{figure}


% The algorithm then iterates to combine nodes into the same community (see Figure~\ref{fig_color}), optimizing the configuration to minimize the total description length. The map equation then evaluates if modularity reaches its maximum when assigning the file object to a different cluster (see Figure~\ref{fig_community}). The algorithm also implicitly optimizes modularity, which is a measure of how well communities separate the network, with good communities having many connections within the community and few connections between communities.

% \begin{figure}[htbp!] 
% \centerline{\includesvg[width=0.40\textwidth]{color.svg}}
% \caption{Flow mapping from introduction phase of CAMEL-789}
% \label{fig_color}
% \end{figure}

% For each dependency graph in each phase originating from ATD items, we calculated the number of nodes, links and leaf nodes. This process was carried out carefully in three main phases: introduction and payment. After obtaining the number of nodes, links and leaf nodes in each phase, we then calculated the delta ($\Delta$) to show the change or difference in the number of nodes, links and leaf nodes from one phase to the next. This delta provides a clear picture of the dynamics of the evolution of the dependency structure of ATD items, which includes how the complexity and interconnectedness in the system change during the life cycle of the items.


% % Number of nodes: 33
% % Number of links: 84
% % Number of leaf nodes: 8
% % Leaf nodes: [12, 23, 10, 26, 13, 29, 30, 21]

% \begin{figure}[htbp!] 
% \centerline{\includesvg[width=0.40\textwidth]{community.svg}}
% \caption{Community detection from introduction phase of CAMEL-789}
% \label{fig_community}
% \end{figure}

\subsubsection{How does the number of changes in files associated with ATD items evolve between the introduction and repayment of the debt?}
To address RQ2, we conducted a comparative study focusing on the change history of files linked to ATD items and non-technical debt items within the project's repository.

We began by identifying 18 ATD items collected from commit messages, issue tracker systems and pull requests. For each ATD item, we determined two key dates:

\begin{itemize}
\item Payment date: We noted the date of the fixing commit that addressed and resolved the ATD item. This date signifies when the technical debt was effectively paid off.

\item Introduction date: Using the \texttt{git blame} tool, we traced each ATD item back to its initial introduction in the codebase. This allowed us to pinpoint the exact commit where the technical debt was first incurred.
\end{itemize}

\textcolor{red}{With both dates established, we calculated the duration of each ATD item—the period during which the technical debt existed in the system. During this timeframe, we analyzed the files associated with each ATD item to assess their modification frequency. Specifically, we extracted the number of commits that involved these files between the introduction and repayment dates to quantify the evolution of changes related to the technical debt.}

\textcolor{red}{To provide a comparative baseline, we randomly selected 18 non-technical debt items from the projects. For these items, we followed similar steps, carefully adjusting terminology to minimize misunderstandings:}

\begin{itemize}
\item Recorded Date: We identified the date when each non-technical debt item was documented or noted in the project records.

\item Initial Commit Date: Using \texttt{git blame}, we traced back to the first commit involving the non-technical debt item to determine when it was first implemented in the codebase.
\end{itemize}

\textcolor{red}{We then calculated the duration between the recorded date and the initial commit date for each non-technical debt item. Within this period, we counted the number of commits involving the associated files to assess their modification frequency, mirroring the approach used for ATD items.}

\textcolor{red}{By comparing the number of changes in files associated with both ATD items and non-ATD items over their respective durations, we aimed to understand the impact of technical debt on code volatility. We investigated whether files linked to ATD items experienced more frequent changes compared to those associated with non-technical debt items, potentially indicating greater instability or increased maintenance efforts due to the presence of technical debt.}

This comparative analysis allowed us to explore patterns in code evolution and assess the extent to which ATD influences the modification frequency of affected files. Understanding these patterns is crucial for identifying areas of the software system that may require additional attention or resources to manage technical debt effectively.


\begin{figure}[htbp!] 
\centerline{\includegraphics[width=0.5\textwidth]{figures/boxplot_number_of_changes.pdf}}
\caption{Boxplot Number of Changes of ATD vs Non-ATD}
\label{fig_number-of-changes}
\end{figure}

The boxplot presented in Figure~\ref{fig_number-of-changes} illustrates the distribution of the number of changes made to the files affected by ATD and non-ATD, from their introduction phase to the payment phase. This analysis provides insights into how frequently these files were modified throughout the lifespan of the technical debt.

The analysis of the ATD items reveals significant variability in the number of changes to files during the lifecycle of technical debt. The mean number of changes per file was 7.13, with a standard deviation of 21.24, indicating that while some files experienced a high number of modifications, others were relatively stable. The median number of changes was 2.0, highlighting that the typical file underwent fewer changes, though certain files acted as hotspots for modifications.


The number of changes ranged from 0 to 811, suggesting that some files with ATD were far more volatile than others. This variability emphasizes that the impact of technical debt is not uniform across files, with a small subset of files requiring significant maintenance efforts during the technical debt period.

We found that some files experienced bursts of high modification activity during their ATD lifecycle. For example, one file underwent as many as 811 changes, while others saw few modifications. These patterns suggest that certain files associated with ATD become areas of concentrated maintenance, reflecting a possible struggle with architectural issues or system dependencies that require repeated adjustments.


%Comparing these findings with non-technical debt items provided a baseline to determine if the observed volatility is indeed attributed to technical debt or is part of normal development activities.

\subsubsection{How does the cyclomatic complexity of code change between the introduction and payment phases of ATD?}
Cyclomatic complexity is a key metric for assessing the structural complexity of code, representing the number of independent paths through a program's control flow. ATD often introduces complexity into the system, which can manifest in various ways, such as increased code branching or convoluted logic. As ATD is resolved, the expectation is that the structural quality of the system improves, potentially reflected by a reduction in cyclomatic complexity.


\subsubsection{Is there a correlation between the number of changes and the cyclomatic complexity of code?}



\begin{figure}[htbp!] 
\centerline{\includegraphics[width=0.5\textwidth]{figures/scatter_plots.pdf}}
\caption{Correlation Between Number of Changes and Cyclomatic Complexity Change}
\label{fig_scatter_plots}
\end{figure}


% \subsection{How does the structure of a dependency graph affect the prioritization of architecture technical debt repayment tasks?}

% \subsection{How is developer involvement in the lifecycle related to the dependency graph structure?}

% %https://refactoring.guru/refactoring
% \begin{table}[htpb]
%     \caption{Code smell types and their descriptions from \cite{martin2003agile, fowler2018refactoring}} 
%     \begin{tabular}{p{2.3cm} p{7.4cm}}
%     \toprule
%     Code smell & Description \\
%     \midrule
%     Data class       & Classes with field and getters and setters not implementing any function in particular        \\
%     Data clumps      & Clumps of data items that are always found together, whether within classes or between classes         \\
%     Duplicated code      & Same or similar code structure repeated within the branches of a conditional statement        \\
%     Feature envy      & A method that seems more interested in others classes than the one it is actually in        \\
%     God class      & A class exhibits the God class if it assumes too many responsibilities compared to its coupled classes, centralizing system functionality in a way that contradicts decomposition design principles        \\
%     God method      & A class exhibits the God method if one of its methods is significantly larger than the others, centralizing the class functionality in a single method        \\
%     Brain class      & Brain class use minimal data from other classes and are typically somewhat more cohesive than God class        \\
%     Brain method      & This smell refers to a large and complex method that centralizes the intelligence of the class        \\
%     Shotgun surgery   & A change in one class necessitates numerous minor adjustments in several other classes        \\
%     Intensive coupling (Inappropriate Intimacy)   & Intensive coupling occurs when methods are heavily interconnected with methods in a few other classes, resulting in excessively verbose communication between the client method and its provider classes        \\
%     Dispersed coupling   & Dispersed coupling, complementary to Intensive coupling, refers to a method excessively tied to many methods across numerous classes, where communication with each class is minimal        \\
%     Primitive obsession   & Overuse of primitive data types instead of small objects for simple tasks        \\
%     Misplaced class &  refers to a class that is in a package that contains other classes not related to it\\
%     %Inappropriate Intimacy  &  \\
    
%     \bottomrule
%     \end{tabular}
%     \label{tab:tb_code_smell}
% \end{table}

==> restructured_main.tex <==
Proposed structure:
1. Introduction
2. Background  

3. Architecture Technical Debt (ATD)  
   (Relevant for theoretical framing.)
4. Dependencies Graph  
   (Part of background; can stay.)
5. The Map Equation  
   (This likely fits with the background.)
6. Methodology  
   - Study Design  
     (Move all aspects of the study process here, including tools, dataset sources, and technologies.)
   - Objectives and Research Questions  
     (Separate clearly from the results.)
7. Results  
   (Only include actual results and analyses related to specific ATD items.)
   - ATD item of CAMEL-789
   - ATD item of CAMEL-4357
   - ATD item of HADOOP-6374
   - Research questions that contain quantitative/qualitative results should move here, avoiding overlap with the methodology.
8. Discussion  
   (Keep as is, ensuring that it summarises and interprets results.)
9. Conclusion  
   (No changes needed here unless requested.)



==> sections/threats.tex <==
\section{Threats to Validity}
\label{sec:_threats}

\subsection{External validity}
The main threat to external validity in this study concerns the generalisability of the findings. As our analysis focused specifically on datasets from selected open-source software (OSS) projects, the results may not extend to proprietary or closed-source systems with different architectural practices, development cultures, or team dynamics. Additionally, the dataset was limited to projects primarily maintained within the Apache ecosystem, potentially limiting the applicability of findings to other OSS communities or development environments. Future studies could address this threat by expanding the sample to include diverse software projects from various domains and development contexts.

\subsection{Internal validity}
One threat to internal validity stems from the selection and re-labelling process used to identify ATD items. Despite rigorous manual validation, potential biases in item selection and labelling may have influenced the final dataset. We counter this threat by only considering the ATD items wher all the raters agreed on the ATD identification of an item. Additionally, focusing exclusively on Violation of Modularity as an ATD indicator, while excluding other forms of architectural debt such as Obsolete Technology, may have limited the comprehensiveness of the analysis. The reliance on specific dependency graph metrics, such as FAN-IN and FAN-OUT, also introduces a risk of measurement bias, as these metrics may not capture all relevant dimensions of ATD impact.

\subsection{Construct validity}
Construct validity threats arise from the metrics and methodologies chosen to assess ATD. FAN-IN and FAN-OUT were used as primary indicators of system connectivity and complexity, however  these metrics may not fully capture the wider architectural implications of ATD, such as modularity, cohesion or code readability. Additionally, our reliance on Natural Language Processing (NLP) techniques for SATD detection may have missed nuanced or implicit expressions of technical debt in developer comments or commit messages, potentially leading to an incomplete dataset. To address these limitations, future research could incorporate a more diverse set of architectural metrics and investigate alternative methods for detecting ATD beyond dependency graphs.

